Robustness Certification for Point Cloud Models

The use of deep 3D point cloud models in safety-critical applications, such as autonomous driving, dictates the need to certify the robustness of these models to real-world transformations. This is technically challenging, as it requires a scalable verifier tailored to point cloud models that handles a wide range of semantic 3D transformations. In this work, we address this challenge and introduce 3DCertify, the first verifier able to certify the robustness of point cloud models. 3DCertify is based on two key insights: (i) a generic relaxation based on first-order Taylor approximations, applicable to any differentiable transformation, and (ii) a precise relaxation for global feature pooling, which is more complex than pointwise activations (e.g., ReLU or sigmoid) but commonly employed in point cloud models. We demonstrate the effectiveness of 3DCertify by performing an extensive evaluation on a wide range of 3D transformations (e.g., rotation, twisting) for both classification and part segmentation tasks. For example, we can certify robustness against rotations by $\pm$60{\deg} for 95.7% of point clouds, and our max pool relaxation increases certification by up to 15.6%.

==> headers/lqa/abbreviations.tex <==
% Description: This file defines commands for common abbreviations
%
% Usage: \input{headers/lqa/abbreviations}

% The Backslash between `.` and ` ` is needed to ensure the white-space is an
% inter-word space, not a inter-sentence space.
%
% Details:
% - https://tex.stackexchange.com/questions/2229/is-a-period-after-an-abbreviation-the-same-as-an-end-of-sentence-period
% - https://stackoverflow.com/questions/2024338/latex-sometimes-puts-too-much-or-too-little-space-after-periods/2024341

\newcommand{\eg}{e.g., }
\newcommand{\ie}{i.e., }
\newcommand{\etc}{etc.}
\newcommand{\cp}{{cp.\ }}
\newcommand{\nth}[1]{$#1^\text{th}$}
\newcommand{\wrt}{{w.r.t.\ }}

==> headers/lqa/colors.tex <==
% Description: This file contains a few useful colors.
%
% Usage: You may need to comment out the usepackage command below, if they
% conflict with your conference template


%%%%%%%%%
% SETUP %
%%%%%%%%%
% import relevant packages

\usepackage[usenames, dvipsnames]{color} % for textcolor
\usepackage{xcolor} % for definecolor


%%%%%%%%%%%%%%%%%%%%%%
%  MATPLOTLIB COLORS %
%%%%%%%%%%%%%%%%%%%%%%


% blue
\definecolor{my-full-blue}{HTML}{1F77B4}
%\definecolor{blue}{RGB}{31,119,180} 

% orange
\definecolor{my-full-orange}{HTML}{FF7F0E}
%\definecolor{orange}{RGB}{255,127,14}

% green
\definecolor{my-full-green}{HTML}{2CA02C}
%\definecolor{green}{RGB}{44,160,44}

% red
\definecolor{my-full-red}{HTML}{d62728}
%\definecolor{red}{RGB}{214,39,40}

% purple
\definecolor{my-full-purple}{HTML}{9467bd}
%\definecolor{purple}{RGB}{148,103,189}

% lighter shades
\colorlet{my-blue}{my-full-blue!30}
\colorlet{my-orange}{my-full-orange!30}
\colorlet{my-green}{my-full-green!30}
\colorlet{my-red}{my-full-red!30}
\colorlet{my-purple}{my-full-purple!30}


%%%%%%%%%%%%%%%%%%%%%%
%  PROJECT-SPECIFIC  %
%%%%%%%%%%%%%%%%%%%%%%
% add project-specific colors here

==> headers/lqa/subfigures.tex <==
% Description: This file introduces a subfigure which correctly aligns
% captions
%
% Usage:
% - \input{headers/lqa/subfigures}
% - You may need to comment out the usepackage command below in case of
%   conflicts

% EXAMPLE USAGE:
%
% \begin{figure}
% 	\centering
% 	\mysubfigure[0.49\linewidth]{
% 		\centering
% 		Content of subfigure 1
% 	}{Caption of subfigure\label{fig:subfig1}}
% 	\mysubfigure[0.49\linewidth]{
% 		\centering
% 		Content of subfigure 2
% 	}{Caption of subfigure\label{fig:subfig2}}
% 	\caption{An example of subfigures.}
% 	\label{fig:subfigures}
% \end{figure}

%%%%%%%%%%%%%%
% USEPACKAGE %
%%%%%%%%%%%%%%
\usepackage{subcaption}

%%%%%%%%%%%
% COMMAND %
%%%%%%%%%%%

\newcommand{\mysubfigure}[3][\linewidth]{\subcaptionbox{#3}[#1]{
	\begin{minipage}{#1}
		% uses minipage to prevent unexpected interactions,
		% e.g., for align
		#2
	\end{minipage}
}}


==> headers/lqa/tikz.tex <==
% Description: This file contains a few useful tikz libraries.
%
% Usage: \input{headers/lqa/tikz}

%%%%%%%%%
% SETUP %
%%%%%%%%%
% import relevant package
\usepackage{tikz}

%%%%%%%%%%%%%%%%%%%%%%
%  PROJECT-SPECIFIC  %
%%%%%%%%%%%%%%%%%%%%%%
% adapt the following list of libraries as required

% \usetikzlibrary{arrows}
% \usetikzlibrary{automata}
% \usetikzlibrary{calc}
% \usetikzlibrary{backgrounds}
% \usetikzlibrary{decorations.markings}
% \usetikzlibrary{decorations.pathmorphing}
% \usetikzlibrary{decorations.pathreplacing}
% \usetikzlibrary{fit}
% \usetikzlibrary{patterns}
% \usetikzlibrary{positioning}
% \usetikzlibrary{shadows}
% \usetikzlibrary{shapes}
% \usetikzlibrary{shapes.geometric}



==> tables/maxpool_perturbation.tex <==
\begin{tabular*}{\columnwidth}{@{}l@{\extracolsep{\fill}}crrcrr@{}}
    \toprule
    && \multicolumn{2}{c}{64 Points} && \multicolumn{2}{c}{128 Points} \\
    \cmidrule{3-4}
    \cmidrule{6-7}
    $\epsilon$ && 0.005 & 0.01 && 0.005 & 0.01 \\
    \midrule
    Boopathy \etal~\cite{boopathy2019cnncert} && 46.7 & 0.0 && 50.5 & 0.0 \\
    DeepPoly~\cite{singh2019abstract} && 81.5 & 15.2 && 82.4 & 5.5 \\
    Ours && \textbf{82.6} & \textbf{22.8} && \textbf{86.8} & \textbf{12.1} \\
    \bottomrule
\end{tabular*}


==> tables/perturbations.tex <==
\begin{tabular*}{\columnwidth}{@{}l@{\extracolsep{\fill}}crrrrr@{}}
    \toprule
    $\epsilon$ && 0.002 & 0.004 & 0.006 & 0.008 & 0.01 \\
    \midrule
    \% Certified && 94.6 & 89.1 & 76.1 & 56.5 & 22.8 \\
    \bottomrule
\end{tabular*}



==> tables/rotation_baseline.tex <==
\begin{tabular}{@{}lrrcrrcrrcrrrcrrrcrr@{}}
    \toprule
    & \multicolumn{8}{c}{No splitting} & \phantom{ab} & \multicolumn{10}{c}{Splitting} \\
    \cmidrule{2-9} \cmidrule{11-20}
    & \multicolumn{2}{c}{$\mathrm{Rot}_{Z}$} && \multicolumn{2}{c}{$\mathrm{Rot}_{ZX}$} && \multicolumn{2}{c}{$\mathrm{Rot}_{ZYX}$} && \multicolumn{3}{c}{$\mathrm{Rot}_{Z}$} && \multicolumn{3}{c}{$\mathrm{Rot}_{ZX}$} && \multicolumn{2}{c}{$\mathrm{Rot}_{ZYX}$} \\
    $\pm \theta$ & 2\textdegree & 3\textdegree && 2\textdegree & 3\textdegree && 1\textdegree & 1.5\textdegree && 10\textdegree & 20\textdegree & 30\textdegree && 3\textdegree & 4\textdegree & 5\textdegree && 2\textdegree & 3\textdegree \\
    \midrule
    Interval & 41.3 & 5.4 && 1.1 & 0.0 && 1.1 & 0.0 && 79.3 & 70.7 & 69.6 && 10.9 & 6.5 & 6.5 && 1.1 & 1.1 \\
    Mohapatra \etal~\cite{mohapatra2020towards} & 43.5 & 6.5 && 1.1 & 0.0 && 1.1 & 0.0 && 85.9 & 84.8 & 80.4 && 13.0 & 12.0 & 10.9 && 1.1 & 1.1 \\
    Ours (DeepG3D) & 96.7 & 93.5 && 32.6 & 2.2 && 73.9 & 8.7 && 97.8 & 96.7 & 95.7 && 94.6 & 91.3 & 89.1 && 72.8 & 64.1 \\
    Ours (Taylor3D) & 96.7 & 93.5 && 32.6 & 2.2 && 73.9 & 8.7 && 97.8 & 96.7 & 95.7 && 94.6 & 91.3 & 89.1 && 69.6 & 63.0 \\
    \bottomrule
\end{tabular}


